Finding Favourite Tuples on Data Streams with Provably Few Comparisons

One of the most fundamental tasks in data science is to assist a user with unknown preferences in finding high-utility tuples within a large database. To accurately elicit the unknown user preferences, a widely-adopted way is by asking the user to compare pairs of tuples. In this paper, we study the problem of identifying one or more high-utility tuples by adaptively receiving user input on a minimum number of pairwise comparisons. We devise a single-pass streaming algorithm, which processes each tuple in the stream at most once, while ensuring that the memory size and the number of requested comparisons are in the worst case logarithmic in $n$, where $n$ is the number of all tuples. An important variant of the problem, which can help to reduce human error in comparisons, is to allow users to declare ties when confronted with pairs of tuples of nearly equal utility. We show that the theoretical guarantees of our method can be maintained for this important problem variant. In addition, we show how to enhance existing pruning techniques in the literature by leveraging powerful tools from mathematical programming. Finally, we systematically evaluate all proposed algorithms over both synthetic and real-life datasets, examine their scalability, and demonstrate their superior performance over existing methods.

==> alg-robust-backup.tex <==
\begin{algorithm}[t]
\DontPrintSemicolon
\KwIn{parameter \Creg}
%\KwOut{Ouput}
$\infd \gets 2, \, R \gets \emptyset, \, S \gets \emptyset$\;

\Function{prune$(\vecx)$}{
	\If{$S \infersim \vecx$ as defined in \cref{eq:implies-robust-backup}}{
		\Return true\;
	}
	\Return false\;
}

\Function{add$(\vecx)$}{
	$S \gets S \cup \{\vecx\}$, and sort \vecx within $R$ \; 
	\eIf{no tie happens}{
		$R \gets R \cup \{\vecx\}$ and create $G_\vecx \gets \{\vecx\}$ \;
	}{
		\For{every $\vecy \in R$ such that $\vecx \cmp \vecy$}{
			$P_\vecx \gets \{ (\vecz,\vecx) \text{ if } \util(\vecz) < \util(\vecx) \text{ else } (\vecx,\vecz) : \vecz \in G_\vecy, \neg (\vecz \cmp \vecx) \}$ \;
			$G_\vecy \gets G_\vecy \cup \{\vecx\}$\;
		}
	}
}

\Function{best$()$}{
	\Return the best tuple in $R$ \;
}

\caption{Another filter for the \irm problem with ties}
\label{alg:robust-backup}
\end{algorithm}

